Learning to Construct 3D Building Wireframes from 3D Line Clouds

Line clouds, though under-investigated in the previous work, potentially encode more compact structural information of buildings than point clouds extracted from multi-view images. In this work, we propose the first network to process line clouds for building wireframe abstraction. The network takes a line cloud as input , i.e., a nonstructural and unordered set of 3D line segments extracted from multi-view images, and outputs a 3D wireframe of the underlying building, which consists of a sparse set of 3D junctions connected by line segments. We observe that a line patch, i.e., a group of neighboring line segments, encodes sufficient contour information to predict the existence and even the 3D position of a potential junction, as well as the likelihood of connectivity between two query junctions. We therefore introduce a two-layer Line-Patch Transformer to extract junctions and connectivities from sampled line patches to form a 3D building wireframe model. We also introduce a synthetic dataset of multi-view images with ground-truth 3D wireframe. We extensively justify that our reconstructed 3D wireframe models significantly improve upon multiple baseline building reconstruction methods. The code and data can be found at https://github.com/Luo1Cheng/LC2WF.

==> header.tex <==
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{booktabs}
% DO NOT USE \usepackage{times}, it will be removed by typesetters
%\usepackage{times}


\usepackage{tikz}
\usepackage{comment}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{xcolor}
\usepackage{color,colortbl}
\input{insbox.tex}
\usepackage{wrapfig}
\usepackage{overpic}
\usepackage[normalem]{ulem}
% INITIAL SUBMISSION - The following two lines are NOT commented
% CAMERA READY - Comment OUT the following two lines
\usepackage{ruler}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

\usepackage{subcaption}
% define some colors for highlights and comments, you can find them on http://latexcolor.com
% blue-ish colors
\definecolor{ao}{rgb}{0.0, 0.0, 1.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\definecolor{celestialblue}{rgb}{0.29, 0.59, 0.82}
\definecolor{azure(colorwheel)}{rgb}{0.0, 0.5, 1.0}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{babyblueeyes}{rgb}{0.63, 0.79, 0.95}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}

% green-ish colors
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}

% purple-ish colors
\definecolor{amethyst}{rgb}{0.6, 0.4, 0.8}
\definecolor{antiquefuchsia}{rgb}{0.57, 0.36, 0.51}
\definecolor{blue-violet}{rgb}{0.54, 0.17, 0.89}
\definecolor{brightlavender}{rgb}{0.75, 0.58, 0.89}
\definecolor{brightube}{rgb}{0.82, 0.62, 0.91}
\definecolor{brilliantlavender}{rgb}{0.96, 0.73, 1.0}

% orange-ish colors
\definecolor{amber}{rgb}{1.0, 0.75, 0.0}
\definecolor{amber(sae/ece)}{rgb}{1.0, 0.49, 0.0}
\definecolor{atomictangerine}{rgb}{1.0, 0.6, 0.4}
\definecolor{burntorange}{rgb}{0.8, 0.33, 0.0}
\definecolor{burntsienna}{rgb}{0.91, 0.45, 0.32}
\definecolor{cadmiumorange}{rgb}{0.93, 0.53, 0.18}
\definecolor{carrotorange}{rgb}{0.93, 0.57, 0.13}
\definecolor{chocolate(web)}{rgb}{0.82, 0.41, 0.12}
\definecolor{chromeyellow}{rgb}{1.0, 0.65, 0.0}
\definecolor{darkorange}{rgb}{1.0, 0.55, 0.0}
\definecolor{darktangerine}{rgb}{1.0, 0.66, 0.07}
\definecolor{deepcarrotorange}{rgb}{0.91, 0.41, 0.17}
\definecolor{deepsaffron}{rgb}{1.0, 0.6, 0.2}
\definecolor{fulvous}{rgb}{0.86, 0.52, 0.0}

\definecolor{tabred}{HTML}{d90429}
\definecolor{tabblue}{HTML}{fb8500}


\newcommand{\TODO}[1]{\textcolor{red}{[TODO: #1]}}
\newcommand{\INSERT}[1]{\textcolor{red}{[INSERT]}}
\newcommand{\CITE}[1]{\textcolor{red}{[CITE]}}
%\newcommand{\revised}[1]{{\color{blue} #1}}

\newcommand{\jing}[1]{\small{\bfseries{\textcolor{orange}{[@jing: #1]}}}}
\newcommand{\xf}[1]{\small{\bfseries{\textcolor{purple}{[@XueFei: #1]}}}}
\newcommand{\kd}[1]{\small{\bfseries{\textcolor{cerulean}{[@KD: #1]}}}}

% \newcommand{\dknote}[1]{\small{\bfseries{\textcolor{cerulean}{[#1]}}}}
% \newcommand{\dk}[1]{\small{\bfseries{\textcolor{ceruleanblue}{#1}}}}
\newcommand{\dk}[1]{\textcolor{ceruleanblue}{#1}}
\newcommand{\dknote}[1]{\small{\bfseries{\textcolor{magenta}{[KD: #1]}}}}

\newcommand{\zxf}[1]{\textcolor{carrotorange}{#1}}


\newcommand{\addref}{\scriptsize{\bfseries{\textcolor{red}{[add ref]}}}}
\newcommand{\todo}[1]{\scriptsize{\bfseries{\textcolor{orange}{[todo: #1]}}}}
\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}


\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}


==> tables/tb_ablation_LPT.tex <==
\centering
\scriptsize
{\def\arraystretch{1.2}\tabcolsep=0.7em
\begin{tabular}{lcccc}
\hline
\toprule[0.8pt]
\textit{LPT Structure} & $\eta=0.15$      & $\eta=0.25$      & $\eta=0.35$      & avg.         \\ \midrule[0.8pt]
ours                          & 90.3/95.2 & \cellcolor{babyblue!15}91.6/96.6 & 92.1/97.2 & \cellcolor{babyblue!15}91.3/96.3 \\ \midrule[0.5pt]
MLP                & 85.0/94.6 &\cellcolor{babyblue!15}86.1/96.2 & 86.6/96.9 & \cellcolor{babyblue!15}85.9/95.9 \\
Single-layer LPT & 86.2/94.7 & \cellcolor{babyblue!15}88.3/96.5 & 89.2/97.2 & \cellcolor{babyblue!15}87.9/96.1 \\ \bottomrule[0.8pt]
\end{tabular}
}



==> tables/tb_ablation_edge_label.tex <==
\centering
\scriptsize
{\def\arraystretch{1.2}\tabcolsep=0.85em
\begin{tabular}{lcccc}
\hline
\toprule[0.8pt]
\textit{Edge Labels} & $\eta=0.15$      & $\eta=0.25$      & $\eta=0.35$      & avg.         \\ \midrule[0.8pt]
5 cate.       & 84.3/91.1 & \cellcolor{babyblue!15}86.9/93.7 & 87.8/94.9 & \cellcolor{babyblue!15}86.3/93.2 \\
2 cate.        & 82.1/91.1  & \cellcolor{babyblue!15}84.7/93.7 & 85.7/94.8   & \cellcolor{babyblue!15}84.2/93.2  \\ \midrule[0.5pt]
5 cate. + post. & 76.8/84.7 & \cellcolor{babyblue!15}80.6/87.1 & 83.9/89.5 & \cellcolor{babyblue!15}80.4/87.1 \\
2 cate. + post.   & 60.4/62.5           & \cellcolor{babyblue!15}64.0/66.1           & 73.5/76.0           & \cellcolor{babyblue!15}65.9/68.5          \\\bottomrule[0.8pt]
\end{tabular}
}



==> tables/tb_ablation_sampling.tex <==
\centering
\scriptsize
{\def\arraystretch{1.2}\tabcolsep=0.6em
\begin{tabular}{lcccc}
\hline
\toprule[0.8pt]
\textit{Sampling Strategy} & $\eta=0.15$      & $\eta=0.25$      & $\eta=0.35$      & avg.         \\ \midrule[0.8pt]
ours                          & 90.3/95.2 & \cellcolor{babyblue!15}91.6/96.6 &
92.1/97.2 & \cellcolor{babyblue!15}91.3/96.3 \\ \midrule[0.5pt]
FPS \textbf{w/out} density                          & 49.4/80.7 & \cellcolor{babyblue!15}58.9/91.2 & 61.7/94.0 & \cellcolor{babyblue!15}56.7/88.6 \\ 
point-to-\textbf{lineSeg}         & 88.1/94.9 & \cellcolor{babyblue!15}89.4/96.4 & 89.9/97.1  & \cellcolor{babyblue!15}89.1/96.1 \\ \bottomrule[0.8pt]
\end{tabular}
}



==> tables/tb_res_direct_output.tex <==
\centering
\scriptsize
{\def\arraystretch{1.2}\tabcolsep=0.65em
\begin{tabular}{lcccccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{} & \multicolumn{2}{c}{output} & \multicolumn{4}{c}{$v\text{AP}_{\eta}$/$v\text{Recall}_{\eta}$  (\%)} & \multicolumn{4}{c}{$s\text{AP}_{\eta}$/$s\text{Recall}_{\eta}$ (\%)} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-11} 
\multicolumn{1}{c}{\multirow{-2}{*}{Method}} & $\vert\mathcal{V}\vert$ & $\vert \mathcal{E} \vert$ & $\eta=0.15$ & $\eta=0.25$ & $\eta=0.35$ & avg. & $\eta=0.25$ & $\eta=0.35$ & $\eta=0.50$ & avg. \\ \midrule[0.8pt]
line3Dpp & 240 & \cellcolor{babyblue!15}120 & 8.90/\textcolor{tabred}{\bfseries 98.1} & \cellcolor{babyblue!15}8.92/\textcolor{tabred}{\bfseries 98.3} & 8.93/\textcolor{tabred}{\bfseries 98.4} & \cellcolor{babyblue!15}8.92/\textcolor{tabred}{\bfseries 98.3} & \textcolor{tabblue}{24.7}/\textcolor{tabblue}{80.8} & \cellcolor{babyblue!15}\textcolor{tabblue}{25.4}/\textcolor{tabblue}{83.0} & \textcolor{tabblue}{25.9}/\textcolor{tabblue}{84.6} & \cellcolor{babyblue!15}\textcolor{tabblue}{25.3}/\textcolor{tabblue}{82.8} \\ \midrule[0.5pt]
line2Surf. & 304 & \cellcolor{babyblue!15}89 & 6.31/88.0 & \cellcolor{babyblue!15}6.45/89.9 & 6.50/90.6 & \cellcolor{babyblue!15}6.42/89.5 & 1.10/27.1 & \cellcolor{babyblue!15}1.15/28.5 & 1.23/30.4 & \cellcolor{babyblue!15}1.16/28.7 \\
PolyFit & 183 & \cellcolor{babyblue!15}250 & 8.99/75.1 & \cellcolor{babyblue!15}10.5/87.6 & 10.8/90.4 & \cellcolor{babyblue!15}10.1/84.4 & 4.16/28.3 & \cellcolor{babyblue!15}5.58/37.9 & 6.56/44.5 & \cellcolor{babyblue!15}5.43/36.9 \\
PC2WF & 69 & \cellcolor{babyblue!15}986 & \textcolor{tabblue}{11.0}/33.2 & \cellcolor{babyblue!15}\textcolor{tabblue}{36.2}/61.3 & \textcolor{tabblue}{46.3}/70.6 & \cellcolor{babyblue!15}\textcolor{tabblue}{31.2}/55.1 & 0.35/14.5 & \cellcolor{babyblue!15}2.86/37.5 & 8.22/58.1 & \cellcolor{babyblue!15}3.81/36.7 \\ \midrule[0.5pt]
\textbf{Ours} & 47 & \cellcolor{babyblue!15}126 & \textcolor{tabred}{\bfseries 91.2}/\textcolor{tabblue}{93.9} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.3}/\textcolor{tabblue}{95.9} & \textcolor{tabred}{\bfseries 93.9}/\textcolor{tabblue}{96.4} & \cellcolor{babyblue!15} \textcolor{tabred}{\bfseries 92.8}/\textcolor{tabblue}{95.4} & \textcolor{tabred}{\bfseries 84.3}/\textcolor{tabred}{\bfseries 90.9} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 86.8}/\textcolor{tabred}{\bfseries 93.4} & \textcolor{tabred}{\bfseries 87.7}/\textcolor{tabred}{\bfseries 94.5} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 86.3}/\textcolor{tabred}{\bfseries 92.9} \\ \bottomrule[0.8pt]
\end{tabular}
}

==> tables/tb_res_postprocess.tex <==
\centering
\tiny
{\def\arraystretch{1.2}\tabcolsep=0.42em
\begin{tabular}{lcccccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{} & \multicolumn{2}{c}{output} & \multicolumn{4}{c}{$v\text{AP}_{\eta}$/$v\text{Recall}_{\eta}$  (\%)} & \multicolumn{4}{c}{$s\text{AP}_{\eta}$/$s\text{Recall}_{\eta}$ (\%)} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-11} 
\multicolumn{1}{c}{\multirow{-2}{*}{Method}} & $\vert\mathcal{V}\vert$ & $\vert \mathcal{E} \vert$ & $\eta=0.15$ & $\eta=0.25$ & $\eta=0.35$ & avg. & $\eta=0.25$ & $\eta=0.35$ & $\eta=0.50$ & avg. \\ \midrule[0.8pt]
line2Surf. & 68 & \cellcolor{babyblue!15}89 & 26.7/\textcolor{tabblue}{83.9} & \cellcolor{babyblue!15}27.4/\textcolor{tabblue}{85.8} & 27.6/86.6 & \cellcolor{babyblue!15}27.2/\textcolor{tabblue}{85.4} & 24.2/\textcolor{tabblue}{58.8} & \cellcolor{babyblue!15}25.1/61.0 & 25.8/62.6 & \cellcolor{babyblue!15}25.0/60.8 \\
PolyFit & 29 & \cellcolor{babyblue!15}43 & \textcolor{tabblue}{52.1}/70.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{62.0}/84.3 & \textcolor{tabblue}{64.3}/\textcolor{tabblue}{87.4} & \cellcolor{babyblue!15}\textcolor{tabblue}{59.5}/80.8 & \textcolor{tabblue}{45.5}/53.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{58.7}/\textcolor{tabblue}{69.5} & \textcolor{tabblue}{65.5}/\textcolor{tabblue}{77.5} & \cellcolor{babyblue!15}\textcolor{tabblue}{56.6}/\textcolor{tabblue}{66.9} \\
PC2WF & 22 & \cellcolor{babyblue!15}34 & 11.9/26.8 & \cellcolor{babyblue!15}43.2/54.3 & 58.5/65.2 & \cellcolor{babyblue!15}37.9/48.8 & 0.84/7.61 & \cellcolor{babyblue!15}7.68/23.3 & 23.0/40.4 & \cellcolor{babyblue!15}10.5/23.8 \\ \midrule[0.5pt]
\textbf{Ours} & 23 & \cellcolor{babyblue!15}39 & \textcolor{tabred}{\bfseries 91.3}/\textcolor{tabred}{\bfseries 92.2} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.4}/\textcolor{tabred}{\bfseries 93.9} & \textcolor{tabred}{\bfseries 94.4}/\textcolor{tabred}{\bfseries 94.8} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.0}/\textcolor{tabred}{\bfseries 93.6} & \textcolor{tabred}{\bfseries 76.8}/\textcolor{tabred}{\bfseries 84.7} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.6}/\textcolor{tabred}{\bfseries 87.1} & \textcolor{tabred}{\bfseries 83.9}/\textcolor{tabred}{\bfseries 89.5} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.4}/\textcolor{tabred}{\bfseries 87.1} \\ \bottomrule[0.8pt]
\end{tabular}
}

==> tables/tb_res_wed.tex <==
\centering
\scriptsize
{\def\arraystretch{1.1}\tabcolsep=0.9em 
\begin{tabular}{lcc|cccccccc}
\toprule[0.8pt]
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{8}{c}{WEDS} \\ \cmidrule(l){4-11} 
\multicolumn{1}{c}{} & \multicolumn{2}{c|}{Topology} & \multicolumn{2}{c}{(WED) \textbf{+vertex}} & \multicolumn{2}{c}{(WED) \textbf{+edge}} & \multicolumn{2}{c}{(WED) \textbf{-edge}} & \multicolumn{2}{c}{(WED) \textbf{Total}} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-11} %\cline{2-11} 
\multicolumn{1}{c}{\multirow{-3}{*}{Method}} & $\vert \mathcal{V} \vert$ & $\vert \mathcal{E} \vert$ & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} \\ \midrule[0.8pt]
\textbf{ground-truth} & 22 $\pm$ 10 & 37 $\pm$ 16 & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- \\ \midrule[0.5pt]
line3Dpp~\cite{Line3Dpp} & 240 $\pm$ 140 & 120 $\pm$ 70 &  0.104 & \cellcolor{babyblue!15} 59.27 & 2.074 & \cellcolor{babyblue!15}8.917 & 49.60 & \cellcolor{babyblue!15}255.7 & 51.77 &  \cellcolor{babyblue!15}323.9 \\ 
Line2Surf.~\cite{surfaceLine} & 68 $\pm$ 68 & 89 $\pm$ 89 & 1.012 & \cellcolor{babyblue!15}13.78 & 6.223 & \cellcolor{babyblue!15}35.76 & 9.427 & \cellcolor{babyblue!15}48.77 & 16.66 & \cellcolor{babyblue!15}98.31 \\
PolyFit~\cite{polyfit} & 29 $\pm$ 15 & 43 $\pm$ 21 & 1.681 & \cellcolor{babyblue!15}3.170 & 4.811 & \cellcolor{babyblue!15}21.41 & {0.969} & \cellcolor{babyblue!15}{5.285} & \textcolor{tabblue}{7.463} & \cellcolor{babyblue!15}\textcolor{tabblue}{29.86} \\
PC2WF~\cite{PC2WF} & 22 $\pm$ 7  & 34 $\pm$ 13 &  5.216 & \cellcolor{babyblue!15}3.445 & 17.01  & \cellcolor{babyblue!15}87.94 & 4.622 & \cellcolor{babyblue!15}33.38 & 26.84  & \cellcolor{babyblue!15}124.8 \\ \midrule[0.5pt]
\textbf{Ours} & 23 $\pm$ 10 & 39 $\pm$ 20 & {0.766} & \cellcolor{babyblue!15}{1.810} & {2.880} & \cellcolor{babyblue!15}{11.49} & 1.655 & \cellcolor{babyblue!15}14.03 & \textcolor{tabred}{\bfseries 5.301} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 27.33} \\ \bottomrule[0.8pt]
\end{tabular}
}







% --------------------------------------------------------
% --- original version (with WED on top)
%---------------------------------------------------------
% \centering
% \tiny
% {\def\arraystretch{1.1}\tabcolsep=0.74em 
% \begin{tabular}{lcc|cccccccc}
% \toprule[0.8pt]
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{8}{c}{WEDS} \\ \cmidrule(l){4-11} 
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\multirow{-2}{*}{Topology}} & \multicolumn{2}{c}{+ vertex} & \multicolumn{2}{c}{+ edge} & \multicolumn{2}{c}{- edge} & \multicolumn{2}{c}{\textbf{Total}} \\ \cmidrule(l){2-11} %\cline{2-11} 
% \multicolumn{1}{c}{\multirow{-3}{*}{Method}} & $\vert \mathcal{V} \vert$ & $\vert \mathcal{E} \vert$ & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} \\ \midrule[0.8pt]
% \textbf{ground-truth} & 22 $\pm$ 10 & 37 $\pm$ 16 & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- \\ \midrule[0.5pt]
% line3Dpp~\cite{Line3Dpp} & 240 $\pm$ 140 & 120 $\pm$ 70 &  0.104 & \cellcolor{babyblue!15} 59.27 & 2.074 & \cellcolor{babyblue!15}8.917 & 49.60 & \cellcolor{babyblue!15}255.7 & 51.77 &  \cellcolor{babyblue!15}323.9 \\ 
% Line2Surf.~\cite{surfaceLine} & 68 $\pm$ 68 & 89 $\pm$ 89 & 1.012 & \cellcolor{babyblue!15}13.78 & 6.223 & \cellcolor{babyblue!15}35.76 & 9.427 & \cellcolor{babyblue!15}48.77 & 16.66 & \cellcolor{babyblue!15}98.31 \\
% PolyFit~\cite{polyfit} & 29 $\pm$ 15 & 43 $\pm$ 21 & 1.681 & \cellcolor{babyblue!15}3.170 & 4.811 & \cellcolor{babyblue!15}21.41 & {0.969} & \cellcolor{babyblue!15}{5.285} & \textcolor{tabblue}{7.463} & \cellcolor{babyblue!15}\textcolor{tabblue}{29.86} \\
% PC2WF~\cite{PC2WF} & 22 $\pm$ 7  & 34 $\pm$ 13 &  5.216 & \cellcolor{babyblue!15}3.445 & 17.01  & \cellcolor{babyblue!15}87.94 & 4.622 & \cellcolor{babyblue!15}33.38 & 26.84  & \cellcolor{babyblue!15}124.8 \\ \midrule[0.5pt]
% \textbf{Ours} & 23 $\pm$ 10 & 39 $\pm$ 20 & {0.766} & \cellcolor{babyblue!15}{1.810} & {2.880} & \cellcolor{babyblue!15}{11.49} & 1.655 & \cellcolor{babyblue!15}14.03 & \textcolor{tabred}{\bfseries 5.301} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 27.33} \\ \bottomrule[0.8pt]
% \end{tabular}
% }

























% \centering
% \scriptsize
% {\def\arraystretch{1.01}\tabcolsep=0.5em 
% \begin{tabular}{lcc|cccccccc}
% \toprule[0.8pt]
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{8}{c}{WEDS} \\ \cmidrule(l){4-11} 
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\multirow{-2}{*}{Topology}} & \multicolumn{2}{c}{+ vertex} & \multicolumn{2}{c}{+ edge} & \multicolumn{2}{c}{- edge} & \multicolumn{2}{c}{Total} \\ \cmidrule(l){2-11} %\cline{2-11} 
% \multicolumn{1}{c}{\multirow{-3}{*}{Method}} & \#vtx & \#edge & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} & Num & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\\ ( m )\end{tabular} \\ \midrule[0.8pt]
% {ground-truth} & 21.81 & 36.85 & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- \\ 
% line3Dpp~\cite{Line3Dpp} & 240.5 & 120.3 &  - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- \\ \midrule[0.5pt]
% Line2Surf~\cite{surfaceLine} & 70.07 & 89.25 & 1.016 & \cellcolor{babyblue!15}13.77 & 6.209 & \cellcolor{babyblue!15}35.63 & 9.604 & \cellcolor{babyblue!15}50.06 & \multicolumn{1}{l}{16.83} & \cellcolor{babyblue!15}99.46 \\
% PolyFit~\cite{polyfit} & 29.71 & 43.62 & 1.681 & \cellcolor{babyblue!15}3.170 & 4.812 & \cellcolor{babyblue!15}21.43 & {0.972} & \cellcolor{babyblue!15}{5.290} & 7.465 & \cellcolor{babyblue!15}29.89 \\
% PC2WF~\cite{PC2WF} & 22.51  & 34.04 &  b3 & \cellcolor{babyblue!15} b4 & b5  & \cellcolor{babyblue!15} b6 & b7 & \cellcolor{babyblue!15} b8 & b9  & \cellcolor{babyblue!15} b10 \\ \midrule[0.5pt]
% {Ours} & 23.73 & 39.03 & {0.766} & \cellcolor{babyblue!15}{1.809} & {2.870} & \cellcolor{babyblue!15}{11.49} & 1.651 & \cellcolor{babyblue!15}14.03 & {5.287} & \cellcolor{babyblue!15}27.33 \\ \bottomrule[0.8pt]
% \end{tabular}
% }





==> tables/tb_suppl_runtime.tex <==
\centering
\scriptsize
{\def\arraystretch{1.2}\tabcolsep=0.65em
\begin{tabular}{lcccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{Method} & \begin{tabular}[c]{@{}c@{}}Data prep.\end{tabular} & \begin{tabular}[c]{@{}c@{}}pre-processing\end{tabular} & \begin{tabular}[c]{@{}c@{}}junc. pred.\end{tabular} & \begin{tabular}[c]{@{}c@{}}edge pred.\end{tabular} & \begin{tabular}[c]{@{}c@{}}plane pred.\end{tabular} & \begin{tabular}[c]{@{}c@{}}surf. recon.\end{tabular} & \begin{tabular}[c]{@{}c@{}}post-processing\end{tabular} & Total \\ \midrule[0.8pt]
line3Dpp & 19.5 & \cellcolor{babyblue!15}13.9 & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}33.1 \\
line2Surf & 33.1 & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & 163.2 & \cellcolor{babyblue!15}57.6 & 0.21 & \cellcolor{babyblue!15}253.9 \\
PolyFit & 63.8 & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & 40.4 & \cellcolor{babyblue!15}5.64 & 0.067 & \cellcolor{babyblue!15}110.0 \\
PC2WF & 63.8 & \cellcolor{babyblue!15}5.21 & 4.94 & \cellcolor{babyblue!15}26.1 & - & \cellcolor{babyblue!15}- & 0.15 & \cellcolor{babyblue!15}100.2 \\ \midrule[0.5pt]
Ours & 19.5 & \cellcolor{babyblue!15}- & 0.18 & \cellcolor{babyblue!15}0.72 & - & \cellcolor{babyblue!15}- & 0.012 & \cellcolor{babyblue!15}20.4 \\ \bottomrule[0.8pt]
\end{tabular}
}

==> tables/useless_rebuttal.tex <==
\centering
\tiny
{\def\arraystretch{1.2}\tabcolsep=0.3em
\begin{tabular}{lcccccccc}
\toprule[0.8pt]
\multicolumn{1}{c}{}  & \multicolumn{4}{c}{$v\text{AP}_{\eta}$/$v\text{Recall}_{\eta}$  (\%)} & \multicolumn{4}{c}{$s\text{AP}_{\eta}$/$s\text{Recall}_{\eta}$ (\%)} \\ \cmidrule(lr){2-5}\cmidrule(lr){6-9} 
\multicolumn{1}{c}{\multirow{-2}{*}{Mtd.}} & $\eta=0.15$ & $\eta=0.25$ & $\eta=0.35$ & avg. & $\eta=0.25$ & $\eta=0.35$ & $\eta=0.50$ & avg. \\ \midrule[0.8pt]
PT & 11.0/33.2 & \cellcolor{babyblue!15}36.2/61.3 & 46.3/70.6 & \cellcolor{babyblue!15}31.2/55.1 & 0.35/14.5 & \cellcolor{babyblue!15}2.86/37.5 & 8.22/\textcolor{tabblue}{58.1} & \cellcolor{babyblue!15}3.81/\textcolor{tabblue}{36.7} \\
PT+p. &  11.9/26.8 & \cellcolor{babyblue!15}43.2/54.3 & 58.5/65.2 & \cellcolor{babyblue!15}37.9/48.8 & 0.84/7.61 & \cellcolor{babyblue!15}7.68/23.3 & 23.0/40.4 & \cellcolor{babyblue!15}10.5/23.8 \\ 
\textcolor{red}{FT} & 17.1/\textcolor{tabblue}{42.4} & \cellcolor{babyblue!15}44.9/\textcolor{tabblue}{71.0} & 53.7/\textcolor{tabblue}{79.2} & \cellcolor{babyblue!15}38.5/\textcolor{tabblue}{64.2} & 1.0/\textcolor{tabblue}{18.8} & \cellcolor{babyblue!15}4.3/\textcolor{tabblue}{38.4} & 7.9/51.9 & \cellcolor{babyblue!15}4.4/36.4 \\
\textcolor{red}{FT+p.}  & \textcolor{tabblue}{18.1}/34.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{52.1}/62.1 & \textcolor{tabblue}{65.6}/71.6 & \cellcolor{babyblue!15}\textcolor{tabblue}{45.3}/56.2 & \textcolor{tabblue}{3.0}/13.4 & \cellcolor{babyblue!15}\textcolor{tabblue}{13.7}/29.8 & \textcolor{tabblue}{26.8}/42.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{14.5}/28.7 \\
\midrule[0.5pt]
\textbf{Ours} & \textcolor{tabred}{\bfseries 91.3}/\textcolor{tabred}{\bfseries 92.2} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.4}/\textcolor{tabred}{\bfseries 93.9} & \textcolor{tabred}{\bfseries 94.4}/\textcolor{tabred}{\bfseries 94.8} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.0}/\textcolor{tabred}{\bfseries 93.6} & \textcolor{tabred}{\bfseries 76.8}/\textcolor{tabred}{\bfseries 84.7} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.6}/\textcolor{tabred}{\bfseries 87.1} & \textcolor{tabred}{\bfseries 83.9}/\textcolor{tabred}{\bfseries 89.5} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.4}/\textcolor{tabred}{\bfseries 87.1} \\ \bottomrule[0.8pt]
\end{tabular}
}



% \centering
% \tiny
% {\def\arraystretch{1.2}\tabcolsep=0.3em
% \begin{tabular}{lcccccccccc}
% \toprule[0.8pt]
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{output} & \multicolumn{4}{c}{$v\text{AP}_{\eta}$/$v\text{Recall}_{\eta}$  (\%)} & \multicolumn{4}{c}{$s\text{AP}_{\eta}$/$s\text{Recall}_{\eta}$ (\%)} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-11} 
% \multicolumn{1}{c}{\multirow{-2}{*}{Mtd.}} & $\vert\mathcal{V}\vert$ & $\vert \mathcal{E} \vert$ & $\eta=0.15$ & $\eta=0.25$ & $\eta=0.35$ & avg. & $\eta=0.25$ & $\eta=0.35$ & $\eta=0.50$ & avg. \\ \midrule[0.8pt]
% PT & 69 & \cellcolor{babyblue!15}986 & 11.0/33.2 & \cellcolor{babyblue!15}36.2/61.3 & 46.3/70.6 & \cellcolor{babyblue!15}31.2/55.1 & 0.35/14.5 & \cellcolor{babyblue!15}2.86/37.5 & 8.22/\textcolor{tabblue}{58.1} & \cellcolor{babyblue!15}3.81/\textcolor{tabblue}{36.7} \\
% PT+p. & 22 & \cellcolor{babyblue!15}34 & 11.9/26.8 & \cellcolor{babyblue!15}43.2/54.3 & 58.5/65.2 & \cellcolor{babyblue!15}37.9/48.8 & 0.84/7.61 & \cellcolor{babyblue!15}7.68/23.3 & 23.0/40.4 & \cellcolor{babyblue!15}10.5/23.8 \\ 
% \textcolor{red}{FT} & 72 & \cellcolor{babyblue!15}321 & 17.1/\textcolor{tabblue}{42.4} & \cellcolor{babyblue!15}44.9/\textcolor{tabblue}{71.0} & 53.7/\textcolor{tabblue}{79.2} & \cellcolor{babyblue!15}38.5/\textcolor{tabblue}{64.2} & 1.0/\textcolor{tabblue}{18.8} & \cellcolor{babyblue!15}4.3/\textcolor{tabblue}{38.4} & 7.9/51.9 & \cellcolor{babyblue!15}4.4/36.4 \\
% \textcolor{red}{FT+p.} & 23 & \cellcolor{babyblue!15}31 & \textcolor{tabblue}{18.1}/34.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{52.1}/62.1 & \textcolor{tabblue}{65.6}/71.6 & \cellcolor{babyblue!15}\textcolor{tabblue}{45.3}/56.2 & \textcolor{tabblue}{3.0}/13.4 & \cellcolor{babyblue!15}\textcolor{tabblue}{13.7}/29.8 & \textcolor{tabblue}{26.8}/42.8 & \cellcolor{babyblue!15}\textcolor{tabblue}{14.5}/28.7 \\
% \midrule[0.5pt]
% \textbf{Ours} & 23 & \cellcolor{babyblue!15}39 & \textcolor{tabred}{\bfseries 91.3}/\textcolor{tabred}{\bfseries 92.2} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.4}/\textcolor{tabred}{\bfseries 93.9} & \textcolor{tabred}{\bfseries 94.4}/\textcolor{tabred}{\bfseries 94.8} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 93.0}/\textcolor{tabred}{\bfseries 93.6} & \textcolor{tabred}{\bfseries 76.8}/\textcolor{tabred}{\bfseries 84.7} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.6}/\textcolor{tabred}{\bfseries 87.1} & \textcolor{tabred}{\bfseries 83.9}/\textcolor{tabred}{\bfseries 89.5} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 80.4}/\textcolor{tabred}{\bfseries 87.1} \\ \bottomrule[0.8pt]
% \end{tabular}
% }

==> tables/useless_rebuttal_2.tex <==
\centering
\tiny
{\def\arraystretch{1.1}\tabcolsep=0.8em 
\begin{tabular}{lcc|cccccccc}
\toprule[0.8pt]
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{} & \multicolumn{8}{c}{WEDS} \\ \cmidrule(l){4-11} 
\multicolumn{1}{c}{} & \multicolumn{2}{c|}{Topology} & \multicolumn{2}{c}{(WED) \textbf{+vertex}} & \multicolumn{2}{c}{(WED) \textbf{+edge}} & \multicolumn{2}{c}{(WED) \textbf{-edge}} & \multicolumn{2}{c}{(WED) \textbf{Total}} \\ \cmidrule(lr){2-3}\cmidrule(lr){4-11} %\cline{2-11} 
\multicolumn{1}{c}{\multirow{-3}{*}{Mtd}} & $\vert \mathcal{V} \vert$ & $\vert \mathcal{E} \vert$ & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\end{tabular} & Num. & \cellcolor{babyblue!15}\begin{tabular}[c]{@{}c@{}}Dist.\end{tabular} \\ \midrule[0.8pt]
% \textbf{ground-truth} & 22 $\pm$ 10 & 37 $\pm$ 16 & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- & - & \cellcolor{babyblue!15}- \\ \midrule[0.5pt]
% line3Dpp~\cite{Line3Dpp} & 240 $\pm$ 140 & 120 $\pm$ 70 &  0.104 & \cellcolor{babyblue!15} 59.27 & 2.074 & \cellcolor{babyblue!15}8.917 & 49.60 & \cellcolor{babyblue!15}255.7 & 51.77 &  \cellcolor{babyblue!15}323.9 \\ 
% Line2Surf.~\cite{surfaceLine} & 68 $\pm$ 68 & 89 $\pm$ 89 & 1.012 & \cellcolor{babyblue!15}13.78 & 6.223 & \cellcolor{babyblue!15}35.76 & 9.427 & \cellcolor{babyblue!15}48.77 & 16.66 & \cellcolor{babyblue!15}98.31 \\
% PolyFit~\cite{polyfit} & 29 $\pm$ 15 & 43 $\pm$ 21 & 1.681 & \cellcolor{babyblue!15}3.170 & 4.811 & \cellcolor{babyblue!15}21.41 & {0.969} & \cellcolor{babyblue!15}{5.285} & \textcolor{tabblue}{7.463} & \cellcolor{babyblue!15}\textcolor{tabblue}{29.86} \\
PT+p. & 22 $\pm$ 7  & 34 $\pm$ 13 &  5.216 & \cellcolor{babyblue!15}3.445 & 17.01  & \cellcolor{babyblue!15}87.94 & 4.622 & \cellcolor{babyblue!15}33.38 & 26.84  & \cellcolor{babyblue!15}124.8 \\
\textcolor{red}{FT+p.} & 23 $\pm$ 8  & 31 $\pm$ 13 &  4.668 & \cellcolor{babyblue!15}3.534 & 18.04  & \cellcolor{babyblue!15}105.73 & 3.843 & \cellcolor{babyblue!15}34.00 & 26.55  & \cellcolor{babyblue!15}143.27 \\
\midrule[0.5pt]
\textbf{Ours} & 23 $\pm$ 10 & 39 $\pm$ 20 & {0.766} & \cellcolor{babyblue!15}{1.810} & {2.880} & \cellcolor{babyblue!15}{11.49} & 1.655 & \cellcolor{babyblue!15}14.03 & \textcolor{tabred}{\bfseries 5.301} & \cellcolor{babyblue!15}\textcolor{tabred}{\bfseries 27.33} \\ \bottomrule[0.8pt]
\end{tabular}
}

==> tables/useless_tb_res_ablation.tex <==

\centering
\scriptsize
{
\begin{tabular}{lllll}
\hline
                              & \multicolumn{4}{c}{\begin{tabular}[c]{@{}c@{}} AP$_{\eta}^{\mathcal{V}}$ / Recall ($\times 10^{-2}$)\\ ($\eta$ has unit of meter)\end{tabular}}                       \\ \hline
                              & $\eta=0.15$      & $\eta=0.15$      & $\eta=0.15$      & avg         \\
fps+density(ours)             & 90.29/95.17 & 91.58/96.58 & 96.58/92.14 & 91.34/96.32 \\
fps                           & 49.41/80.7  & 58.91/91.16 & 61.74/93.96 & 56.71/88.61 \\ \hline
point-to-line segment         & 88.08/94.85 & 89.41/96.44 & 89.89/97.1  & 89.13/96.13 \\ \hline

fps+density(ours)             & 90.29/95.17 & 91.58/96.58 & 96.58/92.14 & 91.34/96.32 \\
ours with mlp                 & 85.01/94.61 & 86.06/96.19 & 86.57/96.93 & 85.88/95.91 \\
ours with one layer attention & 86.23/94.68 & 88.26/96.45 & 89.16/97.16 & 87.88/96.10 \\ \hline
\end{tabular}
}

==> tables/useless_tb_res_ablation2.tex <==
\centering
\scriptsize
{
\begin{tabular}{lllll}
\hline
                      & \multicolumn{4}{c}{sAP/sRecall}                       \\ \cline{2-5} 
                      & n=0.25      & n=0.35      & m=0.5       & avg         \\
five categories       & 84.34/91.14 & 86.85/93.67 & 87.81/94.84 & 86.33/93.21 \\
two categories        & 82.1/91.12  & 84.68/96.66 & 85.7/94.8   & 84.16/93.2  \\ \hline
five with postprocess & 76.78/84.66 & 80.61/87.13 & 83.88/89.48 & 80.42/87.09 \\
two with postprocee   & a           & b           & c           & d          \\ \hline
\end{tabular}

}

==> tables/useless_tb_res_ap.tex <==
\centering
\scriptsize
{\def\arraystretch{1.01}\tabcolsep=0.6em 
\begin{tabular}{lc c c llll}
\toprule[0.8pt]
\multicolumn{1}{c}{} &  &  &  & \multicolumn{4}{c}{} \\
\multicolumn{1}{c}{} &  &  &  & \multicolumn{4}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}} AP$_{\eta}^{\mathcal{V}}$ / Recall ($\times 10^{-2}$)\\ ($\eta$ has unit of meter)\end{tabular}}} \\ \cmidrule(l){5-8} 
\multicolumn{1}{c}{\multirow{-3}{*}{method}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ type\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Output \\ \# vtx\\ (mean $\pm$ std)\end{tabular}} & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average \\ \midrule[0.8pt]
line3Dpp~\cite{Line3Dpp} & \cellcolor{babyblue!20}lines & 1,388 & \cellcolor{babyblue!20}240 $\pm$ 141 & 98.1 & \cellcolor{babyblue!20}98.3 & 98.4 & \cellcolor{babyblue!20}a \\ \midrule[0.5pt]
Line2Surf~\cite{surfaceLine} & \cellcolor{babyblue!20}lines & 120 & \cellcolor{babyblue!20}70.1 $\pm$ 60.9 & 88.0 & \cellcolor{babyblue!20}89.9 & 90.6 & \cellcolor{babyblue!20}b \\
PolyFit~\cite{polyfit} & \cellcolor{babyblue!20}points & 86,396 & \cellcolor{babyblue!20}183 $\pm$ 140 & 75.1 & \cellcolor{babyblue!20}87.6 & 90.4 & \cellcolor{babyblue!20}c \\
PC2WF~\cite{PC2WF} & \cellcolor{babyblue!20}points & 86,396 & \cellcolor{babyblue!20}22.5 $\pm$ 33.7 & 11.5 (35.1) & \cellcolor{babyblue!20}39.2 (66.3) & 50.8 (77.1) & \cellcolor{babyblue!20}d \\ \midrule[0.5pt]
\textbf{Ours} & \cellcolor{babyblue!20}lines & 1,388 & \cellcolor{babyblue!20}23.7 $\pm$ 10.5 & 90.0 (95.5) & \cellcolor{babyblue!20}91.3 (97.0) & 91.9 (97.5) & \cellcolor{babyblue!20}e \\ \bottomrule[0.8pt]
\end{tabular}
}




% \centering
% \scriptsize
% {\def\arraystretch{1.01}\tabcolsep=0.6em 
% \begin{tabular}{lc c c cccc}
% \toprule[0.8pt]
% \multicolumn{1}{c}{} &  &  &  & \multicolumn{4}{c}{} \\
% \multicolumn{1}{c}{} &  &  &  & \multicolumn{4}{c}{\multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}AP$_{\eta}$ / Recall ($\times 10^{-2}$)\\ ($\eta$ has unit of meter)\end{tabular}}} \\ \cmidrule(l){5-8} 
% \multicolumn{1}{c}{\multirow{-3}{*}{method}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ type\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Input\\ size\end{tabular}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Output \\ \# vtx\\ (mean $\pm$ std)\end{tabular}} & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average \\ \midrule[0.8pt]
% line3Dpp~\cite{Line3Dpp} & \cellcolor{babyblue!20}lines & 1,388 & \cellcolor{babyblue!20}240 $\pm$ 141 & 98.1/98.1 & \cellcolor{babyblue!20}98.3/98.3 & 98.4/98.4 & \cellcolor{babyblue!20}a \\
% Line2Surf~\cite{surfaceLine} & \cellcolor{babyblue!20}lines & 120 & \cellcolor{babyblue!20}70.1 $\pm$ 60.9 & 88.0/88.0 & \cellcolor{babyblue!20}89.9/89.9 & 90.6/90.6 & \cellcolor{babyblue!20}b \\
% PolyFit~\cite{polyfit} & \cellcolor{babyblue!20}points & 86,396 & \cellcolor{babyblue!20}183 $\pm$ 140 & 75.1/75.1 & \cellcolor{babyblue!20}87.6/87.6 & 90.4/90.4 & \cellcolor{babyblue!20}c \\
% PC2WF~\cite{PC2WF} & \cellcolor{babyblue!20}points & 86,396 & \cellcolor{babyblue!20}22.5 $\pm$ 33.7 & 11.5/35.1 & \cellcolor{babyblue!20}39.2/66.3 & 50.8/77.1 & \cellcolor{babyblue!20}d \\ \midrule[0.5pt]
% \textbf{Ours} & \cellcolor{babyblue!20}lines & 1,388 & \cellcolor{babyblue!20}23.7 $\pm$ 10.5 & 90.0/95.5 & \cellcolor{babyblue!20}91.3/97.0 & 91.9/97.5 & \cellcolor{babyblue!20}e \\ \bottomrule[0.8pt]
% \end{tabular}
% }


==> tables/useless_tb_res_sap.tex <==
\centering
\scriptsize
{\def\arraystretch{1.01}\tabcolsep=0.2em 
\begin{tabular}{lllllllll}
\toprule[0.8pt]
 & \multicolumn{4}{c}{Before Post-processing} & \multicolumn{4}{c}{After Post-processing} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multirow{-2}{*}{Method} & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average \\ \midrule[0.8pt]
line3Dpp~\cite{Line3Dpp} & - & \cellcolor{babyblue!20}- & - & \cellcolor{babyblue!20}- & 80.8 & \cellcolor{babyblue!20}83.0 & 84.6 & \cellcolor{babyblue!20}j \\ \midrule[0.5pt]
Line2Surf~\cite{surfaceLine} & 27.1 & \cellcolor{babyblue!20}28.5 & 30.4 & \cellcolor{babyblue!20}f & 61.5 & \cellcolor{babyblue!20}63.7 & 65.3 & \cellcolor{babyblue!20}k \\
PolyFit~\cite{polyfit} & 28.3 & \cellcolor{babyblue!20}37.9 & 44.5 & \cellcolor{babyblue!20}g & 53.8 & \cellcolor{babyblue!20}69.5 & 77.5 & \cellcolor{babyblue!20}l \\
PC2WF~\cite{PC2WF} & 0.28 (9.21) & \cellcolor{babyblue!20}3.11 (30.3) & 10.9 (55.1) & \cellcolor{babyblue!20}h & 0.84 (7.61) & \cellcolor{babyblue!20}7.68 (23.3) & 23.0 (40.4) & \cellcolor{babyblue!20}m \\ \midrule[0.5pt]
\textbf{Ours} & 84.3 (91.2) & \cellcolor{babyblue!20}86.9 (93.7) & 87.8 (94.9) & \cellcolor{babyblue!20}i & x & \cellcolor{babyblue!20}y & z & \cellcolor{babyblue!20}h \\ \bottomrule[0.8pt]
\end{tabular}
}




% \centering
% \scriptsize
% {\def\arraystretch{1.01}\tabcolsep=0.4em 
% \begin{tabular}{lcccccccc}
% \toprule[0.8pt]
%  & \multicolumn{4}{c}{Before Post-process} & \multicolumn{4}{c}{After Post-process} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \multirow{-2}{*}{Method} & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average & $\eta=0.15$ & \cellcolor{babyblue!20}$\eta=0.25$ & $\eta=0.35$ & \cellcolor{babyblue!20}average \\ \midrule[0.8pt]
% line3Dpp~\cite{Line3Dpp} & - & \cellcolor{babyblue!20}- & - & \cellcolor{babyblue!20}- & 80.8/80.8 & \cellcolor{babyblue!20}83.0/83.0 & 84.6/84.6 & \cellcolor{babyblue!20}j \\
% Line2Surf~\cite{surfaceLine} & 27.1/27.1 & \cellcolor{babyblue!20}28.5/28.5 & 30.4/30.4 & \cellcolor{babyblue!20}f & 61.5/61.5 & \cellcolor{babyblue!20}63.7/63.7 & 65.3/65.3 & \cellcolor{babyblue!20}k \\
% PolyFit~\cite{polyfit} & 28.3/28.3 & \cellcolor{babyblue!20}37.9/37.9 & 44.5/44.5 & \cellcolor{babyblue!20}g & 53.8/53.8 & \cellcolor{babyblue!20}69.5/69.5 & 77.5/77.5 & \cellcolor{babyblue!20}l \\
% PC2WF~\cite{PC2WF} & 0.28/9.21 & \cellcolor{babyblue!20}3.11/30.3 & 10.9/55.1 & \cellcolor{babyblue!20}h & 0.84/7.61 & \cellcolor{babyblue!20}7.68/23.3 & 23.0/40.4 & \cellcolor{babyblue!20}m \\ \midrule[0.5pt]
% \textbf{Ours} & 84.3/91.2 & \cellcolor{babyblue!20}86.9/93.7 & 87.8/94.9 & \cellcolor{babyblue!20}i & x & \cellcolor{babyblue!20}y & z & \cellcolor{babyblue!20}h \\ \bottomrule[0.8pt]
% \end{tabular}
% }
